Neural Theory-of-Mind? On the Limits of Social Intelligence in Large LMs

Social intelligence and Theory of Mind (ToM), i.e., the ability to reason about the different mental states, intents, and reactions of all people involved, allow humans to effectively navigate and understand everyday social interactions. As NLP systems are used in increasingly complex social situations, their ability to grasp social dynamics becomes crucial. In this work, we examine the open question of social intelligence and Theory of Mind in modern NLP systems from an empirical and theory-based perspective. We show that one of today's largest language models (GPT-3; Brown et al., 2020) lacks this kind of social intelligence out-of-the box, using two tasks: SocialIQa (Sap et al., 2019), which measures models' ability to understand intents and reactions of participants of social interactions, and ToMi (Le et al., 2019), which measures whether models can infer mental states and realities of participants of situations. Our results show that models struggle substantially at these Theory of Mind tasks, with well-below-human accuracies of 55% and 60% on SocialIQa and ToMi, respectively. To conclude, we draw on theories from pragmatics to contextualize this shortcoming of large language models, by examining the limitations stemming from their data, neural architecture, and training paradigms. Challenging the prevalent narrative that only scale is needed, we posit that person-centric NLP approaches might be more effective towards neural Theory of Mind. In our updated version, we also analyze newer instruction tuned and RLFH models for neural ToM. We find that even ChatGPT and GPT-4 do not display emergent Theory of Mind; strikingly even GPT-4 performs only 60% accuracy on the ToMi questions related to mental states and realities.

==> figureTexs/siqa-main.tex <==
\begin{figure*}[t]
     \centering
     \begin{subfigure}[t]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth,trim=3cm 3cm 3cm 3cm]{graphics/SocialIQa-size-k-accuracy-v5.pdf}
         \caption{Accuracy on the \socialIQa dev. set, broken down by \ptlm model type and size, as well as number of few-shot examples ($k$).}
         \label{fig:siqa-acc-by-k-size}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth,trim=3cm 3cm 3cm 3cm]{graphics/SocialIQa-dimsByChar-v4.pdf}
         \caption{Comparing the accuracy of \gptDavinci (35-shot) when the reasoning is about the main agent of the situation versus others. 
        %  \ronan{Can we show that it's not inherently harder? i.e. the human performance doesn't significantly decrease as the focus changes.}\maarten{Unfortunately, I don't have access to the human eval data anymore :(}
         }
         \label{fig:siqa-acc-by-char}
     \end{subfigure}

    \caption{Probing results of several \ptlms on the \socialIQa dev. set.}
    \label{fig:social-iqa-results}
\end{figure*}


==> figureTexs/tomi-main.tex <==
\newcommand{\figHeight}{4.5cm}
\begin{figure*}[t]
     \centering
     

    %  \begin{subfigure}[b]{0.45\textwidth}
    %      \centering
    %      \includegraphics[width=\textwidth,trim=3cm 3cm 2cm 2cm]{graphics/ToMi-acc0vs6shot-v2.pdf}
    %      \caption{Comparing the accuracy of \gptDavinci in a zero-shot setting versus a $k$-shot setting.}
    %      \label{fig:tomi-acc-by-k}
    %  \end{subfigure}
    \begin{subfigure}[t]{0.48\textwidth}
         \centering
         \includegraphics[height=\figHeight,trim=1.5cm 1.5cm 1.5cm 1.45cm,clip]{graphics/ToMi-accByModelSize-mindOnly-v1.pdf}
         \caption{Accuracy on the \tomi dev. set \mind questions of varying sizes of \gptT, and with varying number of examples ($k$).}
         \label{fig:tomi-acc-by-size}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.48\textwidth}
         \centering
         \includegraphics[height=\figHeight,trim=3.5cm 3cm 3cm 2.8cm,clip]{graphics/ToMi-accByMindFactTbFb-v4.pdf}
         \caption{Accuracy of \gptDavinci by number of examples ($k$), by reasoning type (\facts vs. \mind; \mind-\trueBelief vs. \mind-\falseBelief).}
         \label{fig:tomi-acc-by-mind}
     \end{subfigure}
     
    \caption{Probing results of several \ptlms on \tomi.
    \ronan{Maybe we could use the same color code as in Fig. 2}\maarten{I used the \tomi color from Figure 1 (purple) vs. \socialIQa uses the green from Figure 1? but maybe that's dumb and we should keep colors consistent for GPT3-davinci vs ada etc?}
    }
    \label{fig:tomi-results}
\end{figure*}



==> old/2022-05-04-ToMi.tex <==

\newcommand{\memory}{\textsc{Memory}\xspace}
\newcommand{\reality}{\textsc{Reality}\xspace}
\newcommand{\firstorder}{\textsc{First-order}\xspace}
\newcommand{\secondorder}{\textsc{Second-order}\xspace}



\newcommand{\figHeight}{4.2cm}
\begin{figure}[t]
     \centering
     \begin{subfigure}[t]{0.53\textwidth}
         \centering
         \includegraphics[height=\figHeight]{graphics/ToMi-accByExamplesAndSize-1.5k.pdf}
         \caption{Accuracy on the \tomi dev. set, broken down by whether a question requires \ToM to answer and by \ptlm model type and size.}
         \label{fig:siqa-acc-by-size}
     \end{subfigure}
     \hfill
    %  \begin{subfigure}[b]{0.45\textwidth}
    %      \centering
    %      \includegraphics[width=\textwidth,trim=2cm 2cm 2cm 2cm]{graphics/ToMi-acc0vs6shot-v2.pdf}
    %      \caption{Comparing the accuracy of \gptDavinci in a zero-shot setting versus a $k$-shot setting.}
    %      \label{fig:tomi-acc-by-k}
    %  \end{subfigure}
     \begin{subfigure}[t]{0.45\textwidth}
         \centering
         \includegraphics[height=\figHeight]{graphics/ToMi-accByQOrder-1.5k.pdf}
         \caption{Comparing the accuracy of \gptDavinci in a $8$-shot setting, broken down by question \ToM-order (i.e., reasoning type).}
         \label{fig:tomi-acc-by-q-order}
     \end{subfigure}

    \caption{Probing results of several \ptlms on the \socialIQa dev. set.\maarten{Potens: instead of zero- vs. k-shot, do question order tom vs no tom?} \ronan{Maybe we could use the same color code as in Fig. 2}}
    \label{fig:tomi-results}
\end{figure}



Another core component of Theory of Mind is the ability to ascribe mental states and realities to others that are different than one's own.
As a measure of this ability in humans, psychologists developed the \textit{Sally Ann false-belief test} \cite{baron1985does}, in which two people (Sally and Ann) are together in a room with a ball, a basket, and a box, and while Sally is away, Ann moves the ball from the basket to the box.
When asked where Sally will look for her ball, those with \TheoryOfMind are able to guess that Sally will look in the basket (where she left the ball), whereas those without will guess that Sally will look in the box (where the ball is, unbeknownst to Sally).
% To assess whether AI systems could pass this false belief test, \citet{grant2017can} and \citet{nematzadeh2018evaluating} used rule-based logic to create a dataset of such situations.

To measure the false-belief abilities of \ptlms, we use the \tomi QA dataset of Sally-Ann-like stories and questions \cite{le-etal-2019-revisiting}, which is a slightly more challenging version of the rule-based datasets by \citet{nematzadeh2018evaluating} and \citet{grant2017can}.
\tomi stories were created using a stochastic rule-based algorithm that samples two participants, an object of interest, and a set of locations and containers, and weaves together a story (see Table \ref{tab:tomi-examples}).

We investigate how \ptlms answer the \tomi story-question pairs which test for reasoning about mental states,\footnote{The \tomi dataset also generates retrieval questions (e.g., ``\textit{where was the ball originally}'', ``\textit{where is the pen in the end}'') which are much easier to solve and are not the focus of our study.}
of which there are two types:
\firstorder (e.g., ``\textit{where will Sally look for the object?}'') and \secondorder (e.g., ``\textit{where does Sally think that Ann will look for the object?}'').
Both question types can occur with stories where an object was moved either while someone was absent, requiring \ToM to answer, or someone was present, not requiring \ToM to answer.
Each question only has one of two possible answers: the original object location, and the final object location, making this a two-choice QA task.

% \maarten{Update to only focus on the non-reality and non-memory questions}
% By design, there are six types of story-question pairs in \tomi.
% Two are stories with factual questions about the object locations (\memory: ``\textit{where was the object in the beginning?}'' and \reality: ``\textit{where is the object in the end?}'').
% Two are first- and second-order questions for stories where everyone is present when an object is moved (\firstorder: ``\textit{where will Sally look for the object?}'' and \secondorder: ``\textit{where does Sally think that Ann will look for the object?}''), thus requiring no theory of mind.
% Finally, the last two types are first- and second-order questions for stories where the object was moved while someone was absent, which require \ToM to answer correctly.
% Each question only has one of two possible answers: the original object location, and the final object location, making this a two-choice QA task.

%some of the stories involve an object being moved while one of the participants is not present (as with the Sally Ann test), while other stories describe object being moved while both participants are present.
%The questions in \tomi relate to different degrees of \ToM, from simple factual questions (``\textit{where was the object in the beginning?}'' and ``\textit{where is the object in the end?}'') to higher-order \ToM questions (``\textit{where will Sally look for the object?}'' and ``\textit{where does Sally think that Ann will look for the object?}'').
% Additionally, each story-question pair either requires theory-of-mind to answer (e.g., due to someone leaving the location while an object is moved) or does not.

\input{tables/tomi-examples}

\subsection{Probing \ptlms with \tomi}
% To probe our language models, we use the development set of the \socialIQa, which consists of 1,954 QA tuples.
% Following \citet{brown2020language}, we use a $k$-shot language probing setup to obtain predictions.
% Specifically, we concatenate the context ($c$) and question ($q$) together with proper punctuation, and assign the model prediction to the answer ($a_i$, $i\in{1,2,3}$) with the highest conditional likelihood under the language model:
% $$ \argmax_i p_{\text{LM}}(a_i\mid c,q, \mathcal{C}_k)$$
% where $\mathcal{C}_k$ denotes the $k$ training examples, for which we provide the context, question, and correct answer concatenated.

% \paragraph{Experimental Details}
% We vary $k$ from 0 to 35 in increments of 5. As an upper bound of the types of reasoning that the model can do, we select $k$ examples that have the same reasoning dimension.
% We explore model size differences, using the ada (smallest) and two largest (curie, davinci) \gptT models.

% \maarten{Update this (no longer true): We prompt with examples with the same reasoning type (i.e., question order, such as \memory, \firstorder, \secondorder).
% If possible (i.e., for \firstorder and \secondorder story-question pairs), we select 50\% examples that require \ToM to answer, and 50\% that don't.
% Same as before, we explore $k$-shot probing setups, where k is between 0 and 24 (max number of stories that could fit in memory).
% }

As with the previous task, we use the $k$-shot probing setup to test this \ToM component in \ptlms, with $k \in \{2,4,8,16,24\}$.
We select examples of the same reasoning type (i.e., \firstorder or \secondorder), and stratify the examples such that 50\% require \ToM to answer and 50\% do not. 
\maarten{Maybe add some data stats?}
As with \socialIQa, we test \gptAda, \gptCurie, and \gptDavinci.

\subsection{\tomi Results}
Results on \tomi show that all \gptT models substantially struggle with reasoning about mental states, barely reaching 60\% accuracy.
As with \socialIQa, increasing the model size slightly improves the performance (51\% with \gptAda to 60\% with \gptDavinci).
However, contrary to \socialIQa, conditioning on more examples does not seem to yield better accuracy; \gptDavinci reaches its best performance at $k$=8 examples.

Notably, as shown in Fig. \ref{fig:tomi-acc-by-q-order}, the best performing model struggles substantially more with \ToM-questions than with questions that do not require \ToM (XX\% difference).
Additionally, \secondorder questions are harder than \firstorder ones, mirroring how humans struggle with increasingly higher-order \ToM questions \cite{??}.

\maarten{Todo: add a sentence about examples??? or ignore the examples?}

==> old/2022-05-04-tomi-examples.tex <==

\newcommand{\storyColWidth}{7.65cm}
\newcommand{\questionColWidth}{2.05cm}

\newcommand{\firstO}{\textsc{First}}
\newcommand{\secondO}{\textsc{Second}}

\begin{table}[t]
\centering
\footnotesize
%\renewcommand{\arraystretch}{1}
\setlength{\tabcolsep}{3pt}

\begin{tabular}{@{}clll@{}ll@{}}
 \toprule
Order & Story & Question &  &  & Answers \\ \toprule
%  \multirow{4}{\storyColWidth}{Lucas entered the sunroom. Jackson entered the sunroom. Ethan entered the sunroom. The gloves is in the box. Lucas moved the gloves to the treasure chest. Jackson exited the sunroom. Lucas exited the sunroom. Jackson entered the sunroom.} &  \multirow{4}{\questionColWidth}{Where was the gloves at the beginning?} & & & \\
%  & & \personEmoji &  & box \\ 
%  &  &  & \robotEmoji & treasure chest \\
%  &  &  &  &  \\ \midrule
%  \multirow{4}{\storyColWidth}{Isla hates the underclothes. Jayden dislikes the gloves. Isla entered the staircase. William entered the staircase. The raincoat is in the box. William moved the raincoat to the drawer. Isla exited the staircase.} &  \multirow{4}{\questionColWidth}{Where is the raincoat really?} & & & \\
%  & & \personEmoji & \robotEmoji & drawer \\
%  &  &  &  & box \\  &  &  &  &  \\ \midrule


 \multirow{4}{*}{\rotatebox{90}{\firstO}} & \multirow{4}{\storyColWidth}{Benjamin entered the crawlspace. Logan entered the cellar. Avery entered the crawlspace. Logan exited the cellar. The tie is in the cupboard. Avery exited the crawlspace. Benjamin moved the tie to the envelope. Avery entered the cellar.} &  \multirow{4}{\questionColWidth}{Where will Avery look for the tie?} & & & \\
 & & & \personEmoji &  & cupboard \\
 &&   &  & \robotEmoji & envelope \\  &  &  &  &  \\ \midrule

 \multirow{5}{*}{\rotatebox{90}{\secondO}} & \multirow{5}{\storyColWidth}{Emma entered the staircase. William entered the staircase. The lime is in the box. William exited the staircase. Amelia entered the dining room. Emma moved the lime to the cupboard. Emma exited the staircase. Amelia exited the dining room. William entered the dining room.} &  \multirow{5}{\questionColWidth}{Where does Emma think that William searches for the lime?} & & & \\
 & && \personEmoji &  & box \\
 &  &&  & \robotEmoji & cupboard \\  & & &  &  &  \\  & &  &  &  &  \\ \midrule

 \multirow{5}{*}{\rotatebox{90}{\firstO}} & \multirow{5}{\storyColWidth}{James entered the basement. Mia entered the basement. The melon is in the box. James exited the basement. Mia moved the melon to the bucket. Mia exited the basement. Logan entered the workshop. Logan exited the workshop. James entered the workshop.} &  \multirow{5}{\questionColWidth}{Where will James look for the melon?} & & & \\
 & &&  & \robotEmoji & container \\
 &  && \personEmoji &  & drawer \\ &  &&  &  &  \\ &  &  &  &  \\   \midrule 
 
 \multirow{4}{*}{\rotatebox{90}{\secondO}} &
 \multirow{4}{\storyColWidth}{Chloe entered the bedroom. Mia entered the bedroom. The stockings is in the suitcase. Mia exited the bedroom. Mia entered the hall. Jacob dislikes the scarf. Chloe moved the stockings to the treasure chest.} &  \multirow{4}{\questionColWidth}{Where does Mia think that Chloe searches for the stockings?} & & & \\
 & & & &  & treasure chest \\ 
 & &  & \personEmoji & \robotEmoji & suitcase \\  &  &  &  &  \\\bottomrule

\end{tabular}
\caption{Examples of \tomi stories, model predictions, etc.\maarten{todo update to make sure the model actually picked these answers?}}
\label{tab:tomi-examples}
\end{table}

==> old/2022-06-01-discussion.tex <==
\maarten{Comments from IRL meeting:
Frame the discussion more positive, as exciting future directions. How can we bias models towards having ToM? data, arch/representations, training objective
}

\paragraph{\ptlms lack the \TheoryOfMind that humans have}
Our results show that massive pretrained LMs such as \gptT struggle with basic \TheoryOfMind capabilities when used out of the box.
Specifically, \gptT lacks the types of social intelligence and social commonsense needed for the \socialIQa task, where it lags  >30\% humans.
Additionally, \gptT struggles with answering questions about people's mental states and realities, as evidenced by its overall low performance on the \tomi questions about mental states (55-60\%) vs. factual questions (90--100\%).

% Distinguishing Participants: models seem to struggle at representing people, which is a flow that shows up in both tasks.
\paragraph{\ptlms struggle with participant-centric reasoning}
Our analyses also revealed a significant shortcoming of \gptT: its (in)ability to perform participant-centric reasoning about situations.
Results on \socialIQa showed that the model often chooses the answer related to a different character than is asked about, and performs better for questions related to the main character (vs. other, potentially implied, participants).
For \tomi, \gptT performed increasingly worse from factual to first-order to second-order mental state questions.
%Below, we craft two hypotheses to explain these limitations.
Below, we lay out two promising directions that could help bias models towards \TheoryOfMind, focusing on training data and neural architectures.
% worse on questions about participants vs. facts, and worse on second-order than first-order mental state questions.

%\subsection{Training datasets of static text do not display social intelligence}
\subsection{Shifting to training datasets that display social intelligence}
One potential reason for \ptlms's limited social intelligence is the nature of their training data.
Most \ptlms are trained on \textit{static text}, i.e., documents that is written for a general audience and is relatively topically focused and self-contained \cite[e.g., news articles, books, Wikipedia;][]{gao2020pile,dodge2021documentingC4}.
Often, such documents are written such that readers receive most of the information needed, since the content is being communicated exclusively through language.
Readers only require language, world knowledge, and commonsense to interpret such static text \cite{Graesser1994-cc}.

When it comes to learning social commonsense and social intelligence, we posit that the static nature of this text creates certain limitations, through the lens of pragmatics.
First, following Grice's maxim of quantity, static text often omits content that is known by both the author and the reader, to avoid redundancy \cite{grice1975logic}.
\daniel{mention common ground, and cite a Clark paper?}
Also known as reporting bias \cite{Gordon2013reportingbias,Lucy2017AreDR}, this phenomenon hinders the learning of social commonsense knowledge from static text. 
Second, learning to distinguish characters in static text is challenging due to text often having a single focus or perspective. % made challenging by how and when people are referred to by pronouns versus names.
According to Centering Theory \cite{Grosz1995-hm}, the centrality of a character in a discourse is often marked by their being referred to with pronouns, whereas secondary characters are often referred to by name.
% the usage of pronouns for a character in a discourse indicates their centrality, and other characters are then often referred to by their name.
As such, a model trained purely on static text might not learn to resolve coreference for multiple characters inherently \cite{sakaguchi2020winogrande}, much less distinguish mental states and realities of characters.

\maarten{Thus, we argue that different types of data might be needed.
Perhaps grounding in interactional data will be the answer \cite{Bara2021-xd}. 
Or maybe models need to explicitly be taught social intelligence and pronoun resolution in addition to next word prediction.
Additionally, echoing \cite{Bender2020-kt,Bisk2020-xb}, grounding in social context (e.g., social intents) could be helpful to enhance the social intelligence and \TheoryOfMind abilities of these models.
}
\daniel{A couple possible claims: (1) interaction is needed (2) interaction would be helpful (e.g., neural models could learn ToM in the limit, but might learn faster through interaction)}
% . \maarten{Static text, i.e., text that is written for a general audience and is relatively self-contained, such as news articles, books, Wikipedia pages, is often written from an omniscient perspective: the reader receives most of the information needed, since it's content communicated exclusively through language (i.e., it's not often paired with visual or audio media).On the other hand, written text also omits obvious information, such as commonsense, because of grice's maxims.}

% \maarten{
% When it comes to learning about people from static text, Centering Theory \cite{Grosz1995-hm} from pragmatics becomes relevant: often times, we use pronouns for protagonists but use people's names if they are not protagonists. This implies that it may be hard to learn mental state and person-centric realities that are useful for e.g., coref, cause we are often fed the person's name unless it's the protagonist.
% }


% \maarten{Daniel: for the discussion at the end, I wonder if you might consider going position-piece-y and speculating a bit on what interactive data that could help with ToM might look like (e.g., \cite{Bara2021-xd} ?). I don't have any great ideas for this now but would be excited to think about it!  I think this could complement B\&K and Bisk et al which like you said focused less on the social domains.}

% \subsection{Current training objectives and neural architectures are insufficiently person-centric}
\subsection{Exploring person-centric model architectures and training objectives}
.
\maarten{Something about inductive biases for reasoning about 
people more explicitly. Cognitively, we have concept cells \cite{Bowers2017-hp,Calvo_Tapia2020-ll}.
Also, people have made LMs with specific entity representations \cite{Fevry2020-vm,De_Cao2020-ve,Rosset2020-bj}.
Also good to discuss \cite{Langley2022-fl} -- a review discussing ToM and AI (have to read it)
Also, discuss \cite{Wang2022-vi}, they introduce models/tasks that explicitly require ToM, and their model has explicit ToM-ness to it (guessing intentions, etc)
Also cite Yonatan's paper \cite{Zhu2021-zj}, where they explicitly incorporate models of speakers/listeners and show that it helps in speaker-listener games.
Echoing \citet{Bisk2020-xb}, the training objective is also an issue, in that it pushes low-tail things away; perhaps retrieval augmented training or decoding \cite[e.g., kNN-LM, REALM;][]{khandelwal2019generalization,guu2020realm}) should be part of the equation. Or maybe radically new objectives or paradigms are needed.
}
\ronan{We could also include \cite[CALM]{Zhou2021PretrainingTT}, about ``self-supervised pre-training objectives in both generative and contrastive form to improve the commonsense reasoning ability of pre-trained text-to-text transformers''.}


% Specifically we show that these models lag far behind humans ($>$40\%) and behind finetuned models ($>$30\%) on the \socialIQa benchmark, which measure the commonsense reasoning abilities of models with respect to social interactions.

% \maarten{
% We showed that large pretrained LMs such as GPT-3 struggle with basic theory of mind capabilities in few-shot settings.
% Specifically, we show that these models lag far behind humans ($>$40\%) and behind finetuned models ($>$30\%) on the \socialIQa benchmark, which measure the commonsense reasoning abilities of models with respect to social interactions.
% Additionally, using the \tomi dataset, we show models struggle to distinguish between omniscient world knowledge vs. participant-centric world knowledge, lagging far behind human capabilities.
% We discuss some implications of our findings below.
% }

% Something about high-level re-iterating the issues with just pretraining on static language.
% \maarten{
% Limitations of the paradigm of training only on the LM \textit{objective} on static text \textit{data}.
% The issue with the data is that it may not contain enough information about participants, something something centering theory 
% Echoing arguments made by \cite{Bender2020-kt,Bisk2020-xb} on the limitations of learning meaning from pure form only (from pretraining on static text), without grounding in physical or social context.
% } \ronan{+1}




\maarten{Discussion with Ronan: 
(1) static text is typically omniscient narrator perspective, which is what the models probably have the most knowledge of?
(2) probably need to say something about reporting biases and what is ommitted from static text that might be needed to have ToM?
(3) POssibly discuss the strawman of creating a robot-child that learns just from interaction
}

\maarten{Investigate: according to System Error, human brains have roughly 100B neurons , but today's biggest models are almost over that number?? According to further research, there's  100 trillion synapses in the brain which may be a better comparison -- GPT-3 is defs smaller in that case.}

\daniel{Not directly in the scope of the datasets used here, but pragmatic meaning is often derived from reasoning about alternatives -- what the speaker could have said (in another context) but didn't. LLMs don't explicitly get access to these alternatives; they would have to piece them together across contexts.}
\daniel{Other things LLMs don't have access to (but again may be out-of-scope): seeing the perlocutionary effects of language; access to gestures, facial expressions, backchannels, acknowledgements, other features of discourse -- particularly face-to-face discourse -- that indicate uptake or understanding. Cite Clark \& Brennan 1991, or other common grounding literature.}

\daniel{Possible things to call for in future work: intrinsic evaluation / probing of ToM, beyond behavioral evals. Ongoing work has probed for semantics (maybe cite Belinda Li's paper?), which may give a way to ground form-trained models to meaning, while requiring only a very small amount of form--meaning mapping. There are likely analogues of this for pragmatics / ToM.}

\daniel{General ways to get inductive biases in model behavior: encode them in the data, in the architecture, in the loss function, or in intermediate representations. Some of these have been covered above, could there be others? Person-centric data augmentation?}

==> old/2022-06-07-discussion.tex <==
% \maarten{Comments from IRL meeting:
% Frame the discussion more positive, as exciting future directions. How can we bias models towards having ToM? data, arch/representations, training objective
% }
Despite massive successes in other domains, our work highlighted some shortcomings of \ptlms at reasoning about social intelligence and \TheoryOfMind.
Specifically, \gptT's social intelligence as measured by \socialIQa lags behind humans (>30\%), and struggles to answer \tomi questions about mental states (55-60\%) compared factual questions (90--100\%).
We also saw that participant-centric reasoning is a particular challenge for \gptT.
On \socialIQa, it often got participants of situations confused, and performed better for questions related to the main character of situations.
With \tomi, \gptT performed increasingly worse from factual to first-order to second-order mental state questions.
% Below, we discuss pragmatics-informed hypotheses to explain these limitations, as well as some possible future directions to bias models towards \TheoryOfMind.

%Below, we lay out two promising directions that could bias models towards \TheoryOfMind, focusing on training data and neural architectures.

% Our analyses also revealed a significant shortcoming of \gptT: its (in)ability to perform participant-centric reasoning about situations.
% Results on \socialIQa showed that the model often chooses the answer related to a different character than is asked about, and performs better for questions related to the main character (vs. other, potentially implied, participants).
% For \tomi, \gptT performed increasingly worse from factual to first-order to second-order mental state questions.

\subsubsection*{Limitations due to the pragmatics of static text}
%\subsection{Training datasets of static text do not display social intelligence}
%\subsection{Shifting to training datasets that explicitly contain social intelligence}
This limited \TheoryOfMind ability from \ptlms could be explained by examining the training data of \ptlms through a pragmatic lens.
Specifically, most \ptlms are trained on \textit{static text}, which we define as documents that are written for a general audience and are relatively  self-contained and topically focused \cite[e.g., news articles, books, Wikipedia articles;][]{gao2020pile,dodge2021documentingC4}.
Such static text is typically written such that readers only require the language itself as input, which they then combine with their world knowledge and commonsense to understand the text's meaning \cite{Graesser1994-cc}.

When it comes to learning social commonsense and social intelligence, we posit that the static nature of this text creates certain limitations, through the lens of pragmatics.
First, following Grice's maxim of quantity \cite{grice1975logic}, static text often avoids redundancy by omitting content that is known by both the author and the reader \cite{clark1991grounding}.
% \daniel{mention common ground, and cite a Clark paper?}\maarten{good idea, can you try incorporating? \cite{clark1991grounding} }
Also known as reporting bias \cite{Gordon2013reportingbias,Lucy2017AreDR}, this phenomenon hinders the learning of social commonsense knowledge from static text. 
Static text does not include any direct access to \emph{alternative utterances} that the speaker could have chosen to say, but didn't, which are a core component of how people draw pragmatic inferences \cite{grice1975logic,Horn1984-implicature,Levinson2000-implicature}  --- for example, when someone answers \emph{Where does Taylor live?} with \emph{Somewhere in the U.S.}, it likely implicates that they do not know or do not want to share the exact location, since if they did they would have been more specific.
% \maarten{Daniel, can you add a sentence about how static text only contains the ``what happened'' piece of info, not the ``what else could have happened but didn't'' piece, i.e., the alternatives/counterfactuals that you brought up as being an important piece of pragmatics?}

Second, learning to distinguish characters in static text is challenging due to text often having a single focus or perspective. 
According to Centering Theory \cite{Grosz1995-hm}, the centrality of a character in a discourse is often marked by their being referred to with pronouns, whereas secondary characters are often referred to by name.
As such, a model trained purely on static text might not learn to resolve coreference for multiple characters inherently \cite{sakaguchi2020winogrande}, much less distinguish mental states and realities of characters.

Finally, language is primarily learned \cite{wells1981learning,Tomasello2005-intentions} and used \cite{Clark1996-using} in collaborative and interactive settings \cite{Clark1989-discourse}, which allow interlocutors to give immediate feedback to each other on whether their language was understood \cite{Clark2004-monitoring} or should be adjusted \cite{Krauss1966-feedback}, and observe the perlocutionary effects that their language has on their partners \cite{Austin1975-do-things-with-words}.

% \maarten{Potentially, can we make a third but succinct claim about how language primarily used for communication/interaction \cite{wells1981learning}; static text is only one half of the speaker-listener dyad; and interactions allow for immediate feedback of whether what we're saying could/should be ajusted (i.e., perlocutionary aspects of language)? Daniel, if you could give that a go?}

\subsubsection*{Future directions towards \ptlms with \TheoryOfMind}
Due to these limitations, we posit that \ptlms could more efficiently learn \TheoryOfMind abilities through non-static training data, entity-centric neural architectures and social training objectives.
Similar to how visual groundings can help with learning physical knowledge \cite{Zhang2022-nk}, grounding training data in its social context
(e.g., communicative intents, speaker identities) could enable better learning of \TheoryOfMind abilities.
% Echoing arguments by \citet{Bender2020-kt,Bisk2020-xb}, grounding the text used to train \ptlms in its social context (e.g.,  communicative intents, speaker identities) could enable better learning on \TheoryOfMind abilities.
Echoing arguments by \citet{Bender2020-kt,Bisk2020-xb}, this could be accomplished by exploring more interactional training data, such as dialogues in situated contexts \cite{Bara2021-xd,Zhu2021-zj}. 
% \maarten{Challenge is getting this context/metadata then? Can we use the example from \cite{Zhou2021PretrainingTT} as an example that it may be fine to finetune PTLMs on better data to get them to exhibit \TheoryOfMind like abilities better?}

However, changing the training data alone will likely not suffice for \ptlms to efficiently learn social intelligence and \TheoryOfMind; new entity-centric neural architectures are also required.
Humans are believed to have concept cells \cite{Bowers2017-hp,Calvo_Tapia2020-ll}, i.e., sets of neurons that activate for specific people or concepts; we theorize that this type of inductive bias could benefit social intelligence in \ptlms \cite[for a longer discussion of how neurological insights can help with AI \ToM, see][]{Langley2022-fl}.
Prior work has shown that recurrent neural architectures with explicit entity- or person-level representations and training objective can do well at entity identification and tracking tasks \cite{Henaff2017-ov,Ji2017-iq,Yang2017-uk,Liu2019-kn}, and more recent work has corroborated this with larger Transformer-based models \cite{Fevry2020-vm,De_Cao2020-ve,Rosset2020-bj}.
Beyond identification and tracking, \ptlms training could be augmented with tasks specifically related to \TheoryOfMind, such as those explored by \citet{Zhu2021-zj,Wang2022-vi}.

% Additionally, \TheoryOfMind training could be done after an initial pretraining on static text, inspired by promising evidence that pretrained \ptlms better learn commonsense knowledge through additional pretraining on commonsense tasks \cite{Zhou2021PretrainingTT}.
% Such approaches would circumvent the need for augmenting massive corpora of text with social context (e.g., coreference labels, communicative intents).
% % \ronan{We could also include \cite[CALM]{Zhou2021PretrainingTT}, about ``self-supervised pre-training objectives in both generative and contrastive form to improve the commonsense reasoning ability of pre-trained text-to-text transformers''.}

% \maarten{Daniel, can you take a stab at this:}\daniel{Possible things to call for in future work: intrinsic evaluation / probing of ToM, beyond behavioral evals. Ongoing work has probed for semantics (maybe cite Belinda Li's paper \cite{Li2021-mp}), which may give a way to ground form-trained models to meaning, while requiring only a very small amount of form--meaning mapping. There are likely analogues of this for pragmatics / ToM.}

Beyond the data and architecture directions above, alternative training procedures for \ptlms could help produce \TheoryOfMind capabilities.
Recent work has found evidence for latent representations of grounded semantics in models trained only on static text \cite{Li2021-mp}, which can be tied to real-world grounding with a small amount of additional training \cite{Patel2022-mapping}. %. %, \eg in semi-supervised pre-training or in fine-tuning.
Similarly promising experiments show that
% Additionally, \TheoryOfMind training could be done after an initial pretraining on static text, inspired by promising evidence that 
pretrained \ptlms better learn commonsense knowledge through additional pretraining on commonsense tasks \cite{Zhou2021PretrainingTT}.
This latent variable perspective might also help to learn \TheoryOfMind:
we encourage future work to continue to probe for evidence of social and pragmatic representations in existing models, and consider additional human-in-the-loop or multi-agent pre-training and fine-tuning objectives to help surface and strengthen these capabilities, such as those explored by \citet{Hawkins2019-adaptation}, \citet{lazaridou-etal-2020-multi}, \citet{Zhu2021-zj}, and \citet{Wang2022-vi}.
% For theory-of-mind capabilities, 
% Beyond identification and tracking, \ptlms training could be augmented with tasks specifically related to \TheoryOfMind, 
Such approaches might circumvent the need for augmenting massive corpora of text with social context (e.g., coreference labels, communicative intents) while allowing models to learn the \TheoryOfMind capabilities necessary to aid communication and interact successfully with people.


==> old/2022-06-08-introduction.tex <==

% The argument I want to make: LM objective is not enough, we need to incorporate explicit social modeling if we want to get models to do social intelligence. Because LM-ing does not typically require reasoning about many people's mental states

% Something about how Theory of Mind is the ultimate type of reasoning, because it requires mental simulations from all kinds of perspectives.


\section{Introduction}

\begin{figure*}[t]
    \centering
    \includegraphics[width=.95\textwidth]{graphics/IntroFig_v1.pdf}
    \caption{Theory of Mind is the ability for humans to reason about the intents, reactions, and mental states of others. 
    We assess the Theory of Mind abilities of \ptlms through two question answering tasks that measure social commonsense and emotional intelligence (\socialIQa) and reasoning about mental states and false beliefs (\tomi).}
    \label{fig:intro-fig}
\end{figure*}


\textit{\TheoryOfMind} (\ToM), i.e., the ability to infer and reason about the intents, feelings, and mental states of others, is a core component of how humans interact and communicate effectively with each other \cite{Premack1978-sh,apperly2010mindreaders}.
This type of social intelligence allows us, for example, to infer that someone feels boastful after winning a wrestling match (Fig.~\ref{fig:intro-fig}; left). 
Additionally, this ability enables us to reason about other people's mental realities, such as that if someone does not know that a pen was moved while she was out of the room, she will likely search for it where she last saw it instead of where it was moved to (Fig.~ \ref{fig:intro-fig}; right).
% \TheoryOfMind (\ToM) is crucial for humans to navigate everyday encounters; 
With the growing presence of technology in everyday social interactions, 
% As the presence of technology and AI systems in our everyday lives grows,
the need for such \TheoryOfMind and social intelligence in AI systems becomes increasingly necessary \cite{Wang2007-xa,schuller2018age,Dhelim2021-sd}.
% Such \theoryOfMind (\ToM) abilities enable us to 
% seamlessly navigate social situations ranging from friendly interactions to complex negotiations \cite{apperly2010mindreaders}.
% seamlessly navigate everyday encounters \cite{apperly2010mindreaders}.
% and is increasingly necessary for AI systems to successfully interface or interact with us in our everyday lives \cite{Wang2007-xa,Pereira2016socialpower,schuller2018age}.
% As AI systems are increasingly prevalent in everyday lives, such \ToM abilities in these systems are going to become increasingly necessary. 
%\maarten{Short paragraph describing the two types of social intelligence we refer to (e.g., commonsense reasoning about social interaction, false belief tests}

\maarten{Maybe more position-y: In this work, we discuss why \ToM and social commonsense reasoning remain an elusive goal, }
In this work, we establish that \ToM and social commonsense reasoning remains an elusive goal for modern AI systems such as large neural language models (\ptlms)\maarten{, despite suggestions that these models are capable of commonsense reasoning \cite{Narang2022palmsBlog}?}.
With advances in scaling the model sizes and training datasets, these \ptlms have proven very impressive at generating human-like language for conversational, summarization, or sentence continuation settings, often with none to few examples to learn from \cite{brown2020language,clark2021all,Chowdhery2022palm}.
% We investigate to what extent such \ToM abilities remain a challenge for modern AI systems such as large neural language models (\ptlms).
% Recent advances \ptlms due to scaling the training data and model size have made these models quite impressive at things like conversations, summarization, etc. often with no or few training examples \cite{brown2020language,clark2021all}.
However, increasing scrutiny has shed light onto the shortcomings of these \ptlms, showing that they often fall prey to spurious correlational patterns instead of displaying higher-order reasoning behavior \cite{Bender2020-kt,Bisk2020-xb,elkins2020can,dale2021gpt,Marcus2022-fg}.
% coherence, commonsense, factuality, or consistency
%However, there is increasing discourse/evidence that these models lack fundamental social reasoning abilities \cite{Bender2020-kt,Bisk2020-xb,elkins2020can,dale2021gpt,somethingEmpirical}.
%\maarten{Paragraph/sentence about why AI systems need this kind of intelligence? they are increasingly prevalent in society, increasingly engaged in social tasks like communication\cite{Chen2019smartCompose}, counseling \cite{Kearns2020-ty,Allen2020-cd}, educational settings \cite{breazeal2002designing,williams2019popbots}}


% \maarten{Argument: PTLMs have gotten super super good at so many tasks, like conversational }
% Despite impressive advances in neural modelling, this type of complex social reasoning remains a challenge for modern AI systems such as large neural language models (\ptlms).

We show that out-of-the-box \ptlms struggle at two types of reasoning abilities that are requisites for \TheoryOfMind (shown in Fig.~\ref{fig:intro-fig}), using some of the largest \ptlms in existence \cite[\gptT;][]{brown2020language}.
% We show that out-of-the-box large LMs (\ptlms) such as \gptT \cite{brown2020language} severely lack these abilities, showing that they struggle on two \TheoryOfMind tasks.
The first task assesses whether \ptlms can reason about \textit{social commonsense and emotional intelligence} with respect to social situations (\S\ref{sec:socialIQa}), using the \socialIQa benchmark \cite{sap2019socialIQa} illustrated in Fig. \ref{fig:intro-fig} (left).
Our best performing few-shot \gptT setup achieves only 55\% accuracy on this 3-way QA benchmark, lagging $>$30\% behind human performance.
Furthermore, social reasoning about the protagonists of situations is easier for \gptT (5-15\% absolute difference) compared to reasoning about other secondary participants.

Our second task uses the \tomi benchmark \cite{le-etal-2019-revisiting} to measure \ptlms' ability to \textit{understand other people's mental states and realities} in short stories (\S\ref{sec:ToMi}; illustrated in Fig. \ref{fig:intro-fig}; right), inspired by the classic Sally-Ann False Belief \TheoryOfMind test \cite{baron1985does}.
% , this benchmark contains stories about people and objects, along with questions about where an object is located (either in reality or where people think
Our results show that \gptT models peak at 60\% accuracy on questions about participants' mental states, compared to 90--100\% on factual questions.
% \maarten{Unclear that we need this extra sentence?}
% Surprisingly, \gptT appears equally puzzled by questions about people's mental states that require \ToM (i.e., false beliefs) vs. that require no \ToM to answer (i.e., true beliefs).
% Our results show that \gptT models perform 10-15\% worse than random chance on questions that require \ToM reasoning about false beliefs, despite being able to answer non-\ToM questions with reasonable performance.
% Surprisingly, we find that as \gptT models grow larger, their performance difference on questions that require \ToM and don't increases \ronan{not so clear}, compared to smaller models that are generally closer to random performance.

Our work presents a novel exploration of \gptT's abilities to perform \theoryOfMind reasoning, showing that reasoning about social situations and false beliefs still presents a significant challenge for large language models.
In \S\ref{sec:discussion-conclusion}, we discuss the implications of these findings, highlighting the limitations of the current language modelling paradigm on general audience ``static'' text. 
Echoing several others \cite{Bender2020-kt,Bisk2020-xb}, we postulate that in order to achieve better neural \TheoryOfMind, interaction-grounded or entity-centric approaches will likely be necessary.
\maarten{Maybe instead say something about how we frame the limitations through a pragmatics lens, and echo ...}

% Large language models are increasingly used in user-facing settings to enable communication (e.g., email writing, counseling).
% These skills require the ability to understand that there are multiple participants in situations, each of which has their own perception of reality and their own set of intents and emotions.
% \maarten{Refer to a figure 1 if we make one}



% Writing emails or online text: https://techcrunch.com/2020/11/12/othersideai-raises-2-6m-to-let-gpt-3-write-your-emails-for-you/
% 


==> old/2022-06-15-discussion.tex <==
% \maarten{Comments from IRL meeting:
% Frame the discussion more positive, as exciting future directions. How can we bias models towards having ToM? data, arch/representations, training objective
% }
Despite massive successes in other domains, our work highlighted some shortcomings of \ptlms at reasoning about social intelligence and \TheoryOfMind.
Specifically, \gptT's social intelligence as measured by \socialIQa lags behind humans (>30\%), and struggles to answer \tomi questions about mental states (55-60\%) compared factual questions (90--100\%).
We also saw that participant-centric reasoning is a particular challenge for \gptT.
On \socialIQa, it often got participants of situations confused, and performed better for questions related to the main character of situations.
With \tomi, \gptT performed increasingly worse from factual to first-order to second-order mental state questions.
% Below, we discuss pragmatics-informed hypotheses to explain these limitations, as well as some possible future directions to bias models towards \TheoryOfMind.

%Below, we lay out two promising directions that could bias models towards \TheoryOfMind, focusing on training data and neural architectures.

% Our analyses also revealed a significant shortcoming of \gptT: its (in)ability to perform participant-centric reasoning about situations.
% Results on \socialIQa showed that the model often chooses the answer related to a different character than is asked about, and performs better for questions related to the main character (vs. other, potentially implied, participants).
% For \tomi, \gptT performed increasingly worse from factual to first-order to second-order mental state questions.

\subsubsection*{Limitations due to the pragmatics of static text}
%\subsection{Training datasets of static text do not display social intelligence}
%\subsection{Shifting to training datasets that explicitly contain social intelligence}
This limited \TheoryOfMind ability from \ptlms could be explained by examining the training data of \ptlms through a pragmatic lens.
Specifically, most \ptlms are trained on \textit{static text}, which we define as documents that are written for a general audience and are relatively  self-contained and topically focused \cite[e.g., news articles, books, Wikipedia articles;][]{gao2020pile,dodge2021documentingC4}.
Such static text is typically written such that readers only require the language itself as input, which they then combine with their world knowledge and commonsense to understand the text's meaning \cite{Graesser1994-cc}.

When it comes to learning social commonsense and social intelligence, we posit that the static nature of this text creates certain limitations, through the lens of pragmatics.
First, following Grice's maxim of quantity \cite{grice1975logic}, static text often avoids redundancy by omitting content that is known by both the author and the reader \cite{clark1991grounding}.
% \daniel{mention common ground, and cite a Clark paper?}\maarten{good idea, can you try incorporating? \cite{clark1991grounding} }
Also known as reporting bias \cite{Gordon2013reportingbias,Lucy2017AreDR}, this phenomenon hinders the learning of social commonsense knowledge from static text. 
Static text does not include any direct access to \emph{alternative utterances} that the speaker could have chosen to say, but didn't, which are a core component of how people draw pragmatic inferences \cite{grice1975logic,Horn1984-implicature,Levinson2000-implicature}  --- for example, when someone answers \emph{Where does Taylor live?} with \emph{Somewhere in the U.S.}, it likely implicates that they do not know or do not want to share the exact location, since if they did they would have been more specific.
% \maarten{Daniel, can you add a sentence about how static text only contains the ``what happened'' piece of info, not the ``what else could have happened but didn't'' piece, i.e., the alternatives/counterfactuals that you brought up as being an important piece of pragmatics?}

Second, learning to distinguish characters in static text is challenging due to text often having a single focus or perspective. 
According to Centering Theory \cite{Grosz1995-hm}, the centrality of a character in a discourse is often marked by their being referred to with pronouns, whereas secondary characters are often referred to by name.
As such, a model trained purely on static text might not learn to resolve coreference for multiple characters inherently \cite{sakaguchi2020winogrande}, much less distinguish mental states and realities of characters.

Finally, language is primarily learned \cite{wells1981learning,Tomasello2005-intentions} and used \cite{Clark1996-using} in collaborative and interactive settings \cite{Clark1989-discourse}, which allow interlocutors to give immediate feedback to each other on whether their language was understood \cite{Clark2004-monitoring} or should be adjusted \cite{Krauss1966-feedback}, and observe the perlocutionary effects that their language has on their partners \cite{Austin1975-do-things-with-words}.

% \maarten{Potentially, can we make a third but succinct claim about how language primarily used for communication/interaction \cite{wells1981learning}; static text is only one half of the speaker-listener dyad; and interactions allow for immediate feedback of whether what we're saying could/should be ajusted (i.e., perlocutionary aspects of language)? Daniel, if you could give that a go?}

\subsubsection*{Future directions towards \ptlms with \TheoryOfMind}
Due to these limitations, we posit that \ptlms could more efficiently learn \TheoryOfMind abilities through non-static training data, entity-centric neural architectures and social training objectives.
Similar to how visual groundings can help with learning physical knowledge \cite{Zhang2022-nk}, grounding training data in its social context
(e.g., communicative intents, speaker identities) could enable better learning of \TheoryOfMind abilities.
% Echoing arguments by \citet{Bender2020-kt,Bisk2020-xb}, grounding the text used to train \ptlms in its social context (e.g.,  communicative intents, speaker identities) could enable better learning on \TheoryOfMind abilities.
Echoing arguments by \citet{Bender2020-kt,Bisk2020-xb}, this could be accomplished by exploring more interactional training data, such as dialogues in situated contexts \cite{Bara2021-xd,Zhu2021-zj}. 
% \maarten{Challenge is getting this context/metadata then? Can we use the example from \cite{Zhou2021PretrainingTT} as an example that it may be fine to finetune PTLMs on better data to get them to exhibit \TheoryOfMind like abilities better?}

However, changing the training data alone will likely not suffice for \ptlms to efficiently learn social intelligence and \TheoryOfMind; new entity-centric neural architectures are also required.
Humans are believed to have concept cells \cite{Bowers2017-hp,Calvo_Tapia2020-ll}, i.e., sets of neurons that activate for specific people or concepts; we theorize that this type of inductive bias could benefit social intelligence in \ptlms \cite[for a longer discussion of how neurological insights can help with AI \ToM, see][]{Langley2022-fl}.
Prior work has shown that recurrent neural architectures with explicit entity- or person-level representations and training objective can do well at entity identification and tracking tasks \cite{Henaff2017-ov,Ji2017-iq,Yang2017-uk,Liu2019-kn}, and more recent work has corroborated this with larger Transformer-based models \cite{Fevry2020-vm,De_Cao2020-ve,Rosset2020-bj}.
Beyond identification and tracking, \ptlms training could be augmented with tasks specifically related to \TheoryOfMind, such as those explored by \citet{Zhu2021-zj,Wang2022-vi}.

% Additionally, \TheoryOfMind training could be done after an initial pretraining on static text, inspired by promising evidence that pretrained \ptlms better learn commonsense knowledge through additional pretraining on commonsense tasks \cite{Zhou2021PretrainingTT}.
% Such approaches would circumvent the need for augmenting massive corpora of text with social context (e.g., coreference labels, communicative intents).
% % \ronan{We could also include \cite[CALM]{Zhou2021PretrainingTT}, about ``self-supervised pre-training objectives in both generative and contrastive form to improve the commonsense reasoning ability of pre-trained text-to-text transformers''.}

% \maarten{Daniel, can you take a stab at this:}\daniel{Possible things to call for in future work: intrinsic evaluation / probing of ToM, beyond behavioral evals. Ongoing work has probed for semantics (maybe cite Belinda Li's paper \cite{Li2021-mp}), which may give a way to ground form-trained models to meaning, while requiring only a very small amount of form--meaning mapping. There are likely analogues of this for pragmatics / ToM.}

Beyond the data and architecture directions above, alternative training procedures for \ptlms could help produce \TheoryOfMind capabilities.
Recent work has found evidence for latent representations of grounded semantics in models trained only on static text \cite{Li2021-mp}, which can be tied to real-world grounding with a small amount of additional training \cite{Patel2022-mapping}. %. %, \eg in semi-supervised pre-training or in fine-tuning.
Similarly promising experiments show that
% Additionally, \TheoryOfMind training could be done after an initial pretraining on static text, inspired by promising evidence that 
pretrained \ptlms better learn commonsense knowledge through additional pretraining on commonsense tasks \cite{Zhou2021PretrainingTT}.
This latent variable perspective might also help to learn \TheoryOfMind:
we encourage future work to continue to probe for evidence of social and pragmatic representations in existing models, and consider additional human-in-the-loop or multi-agent pre-training and fine-tuning objectives to help surface and strengthen these capabilities, such as those explored by \citet{Hawkins2019-adaptation}, \citet{lazaridou-etal-2020-multi}, \citet{Zhu2021-zj}, and \citet{Wang2022-vi}.
% For theory-of-mind capabilities, 
% Beyond identification and tracking, \ptlms training could be augmented with tasks specifically related to \TheoryOfMind, 
Such approaches might circumvent the need for augmenting massive corpora of text with social context (e.g., coreference labels, communicative intents) while allowing models to learn the \TheoryOfMind capabilities necessary to aid communication and interact successfully with people.


==> old/2022-06-20-discussion.tex <==
% \maarten{Comments from IRL meeting:
% Frame the discussion more positive, as exciting future directions. How can we bias models towards having ToM? data, arch/representations, training objective
% }

Most humans develop social intelligence and \TheoryOfMind naturally.
However, in this work, we showed that these abilities do not emerge automatically in large-pretrained language models. 
These shortcomings contrast with the wealth of successes of \ptlms at a variety of tasks, including tasks that potentially require social intelligence. 
For example, \gptT has been shown to generate stories with emotional arcs that are virtually indistinguishable from human-written stories \cite{clark2021all}.
Additionally, recent work has used \gptT to generate social commonsense knowledge related to protagonists of situations \cite{west2022symbolic}.
While those findings suggest some level of social and emotional intelligence in \ptlms, our explorations highlight the limits of these abilities, and raise the open question: \textit{how can we create NLP systems with true social intelligence and \TheoryOfMind?}

To begin answering this question, we first discuss the current \ptlms training paradigm (\S\ref{ssec:limitations-of-paradigm}), drawing from pragmatics theories to examine why these models are not learning social intelligence efficiently.
Then, we outline some possible future directions to bias models towards \TheoryOfMind (\S\ref{ssec:future-directions}), through person-centric neural architectures, data selection, and training objectives.
% discuss pragmatics-informed hypotheses to explain these limitations, as well as some possible future directions to bias models towards \TheoryOfMind.

% \maarten{Focus on how social intelligence is a goal, maybe re-iterate some of the points from section 2 about how this is going to be necessary. Then discuss why this limitation is showing up;
% It's obvious that LMs should have social intelligence, and need to discuss that they kind of do things that require social intelligence already. However, there are still some big missing gaps.}

% conclusion paragraph, summarizing the findings briefly

% pop higher level, describe that these conclusions could be somewhat surprising in light of recent successes of PTLMs at tasks that seem quite social intelligence related

% reiterate that true social intelligence is needed, and that there are some fundamental limitations 



% Despite massive successes in other domains, our work highlighted some shortcomings of \ptlms at reasoning about social intelligence and \TheoryOfMind.
% Specifically, \gptT's social intelligence as measured by \socialIQa lags behind humans (>30\%), and struggles to answer \tomi questions about mental states (55-60\%) compared factual questions (90--100\%).
% We also saw that participant-centric reasoning is a particular challenge for \gptT.
% On \socialIQa, it often got participants of situations confused, and performed better for questions related to the main character of situations.
% With \tomi, \gptT performed increasingly worse from factual to first-order to second-order mental state questions.

\newcommand{\static}{static\xspace}
\newcommand{\Static}{Static\xspace}


\subsection{The Pragmatics of ``\Static'' Text}
\label{ssec:limitations-of-paradigm}
To understand why \ptlms are still struggling with social intelligence and \TheoryOfMind, we examine \ptlms' training paradigm through the lens of \textit{pragmatics}.
As discussed in \S\ref{sec:background}, pragmatics provides a connection between language development and \TheoryOfMind \cite{Sperber1986-ha,Miller2006-pg,Tauzin2018-na}: learning to communicate effectively with language requires reasoning about what our interlocutor knows or does not know \cite{grice1975logic,Fernandez2013-su,Goodman2016-rsa,Enrici2019-mf}.\footnote{
Note here that, in contrast to other work \cite{Bender2020-kt,Bisk2020-xb}, we do not focus on whether \ptlms ``understand'' language, instead we examine whether \ptlms can answer questions about the emotions and mental states of participants of situations.}

% This limited \TheoryOfMind ability from \ptlms could be explained by examining \ptlms' training data of through a pragmatic lens.
% Specifically, 
Humans' predominant use of language is to communicate about relationship and personal experiences \cite{Clark1989-discourse,Dunbar1993-ew}.
This is fundamentally different from the training data of \ptlms, which consists of language found in what we call \textit{\static} texts: documents that are written for a general audience and are relatively self-contained and topically focused \cite[e.g., news articles, books, Wikipedia articles;][]{gao2020pile,dodge2021documentingC4}.
\daniel{I like that \emph{\static} is concise, but I don't feel it captures all the limitations that we're outlining here. I also feel that general audience and topically focused don't exclude the other things we lay out - eg you could imagine topically focused/general audience conversations that have most/all of the features below. Maybe something like \emph{observational}, or \emph{egocentric}, or \emph{non-social}?} \maarten{How about ``unidirectional''?}
% Most \ptlms are trained on \textit{\static} text, which we define as documents that are written for a general audience and are relatively  self-contained and topically focused \cite[e.g., news articles, books, Wikipedia articles;][]{gao2020pile,dodge2021documentingC4}.
Such \static text is typically written such that readers only require the language itself as input, which they then combine with their world knowledge and commonsense to understand its meaning \cite{Graesser1994-cc}.

If AI systems are to learn social intelligence and \TheoryOfMind, we posit that \static text has certain limitations, from a pragmatics lens, outlined below. %  We outline those below.
% When it comes to learning social commonsense and social intelligence, we posit that the \static nature of this text creates certain limitations, through the lens of pragmatics.

\paragraph{Reporting bias.}
Following Grice's maxim of quantity \cite{grice1975logic}, \static text often avoids redundancy by omitting content that is known by both the author and the reader \cite{clark1991grounding}.
% \daniel{mention common ground, and cite a Clark paper?}\maarten{good idea, can you try incorporating? \cite{clark1991grounding} }
Also known as reporting bias \cite{Gordon2013reportingbias,Lucy2017AreDR}, this phenomenon likely hinders the learning of social commonsense knowledge from \static text, including for \ptlms.

% \paragraph{Lack of alternatives.}
\paragraph{Lack of communicative intent and alternatives.}
% \daniel{Thinking about this more in conjunction with another paper, I'm inclined to change this to change this to \emph{lack of communicative intent}, but still use the same examples we have (and end in the same way).}\maarten{I see your point, but wondering how to describe these concepts in this context... Tried below}
A corollary to reporting bias, \static text does not provide any direct access to \textit{communicative intent} (why words were used) or to \textit{alternatives} (which words were not used, and why).
% A corollary to reporting bias, \static text does not provide any direct access to \textit{alternative utterances} that the author could have chosen to write, but did not.
This reasoning about intents, alternatives, and their implications is
% which are 
a core component of how people draw pragmatic inferences about their interlocutor's mental states \cite{grice1975logic,Horn1984-implicature,Levinson2000-implicature}  --- for example, when someone answers \emph{Where does Taylor live?} with \emph{Somewhere in the U.S.}, it implies that they likely do not know or do not want to share the exact location, since, if they did, they would have been more specific.
% \maarten{Tried to add a sentence about how that could affect models, Daniel plz double check}
This poses a likely limitation that \ptlms only learn what words are used, but not which words were not used, and why.
% \maarten{One sentence about how this could affect models?}
% \maarten{Daniel, can you add a sentence about how \static text only contains the ``what happened'' piece of info, not the ``what else could have happened but didn't'' piece, i.e., the alternatives/counterfactuals that you brought up as being an important piece of pragmatics?}


\paragraph{Lack of communicative effects.} % \maarten{Daniel please double check that I'm using backchannel properly?}
% \daniel{perhaps change this to \emph{lack of communicative effects}. This would be a bit more general --- backchannel is one specific way that communicative effects are conveyed but there are others. It would also parallel the proposed structure for para 2 (could also reorder paras to put these next to each other)}\maarten{Done, sounds good!}
Language is primarily learned \cite{wells1981learning,Tomasello2005-intentions} and used \cite{Clark1996-using} in collaborative and interactive settings \cite{Clark1989-discourse}, which allow interlocutors to backchannel, i.e., give immediate feedback to each other on whether their language was understood \cite{Clark2004-monitoring} or should be adjusted \cite{Krauss1966-feedback}, and observe the perlocutionary effects that their language has on their partners \cite{Austin1975-do-things-with-words}.
\maarten{Again, tried to add a sentence about how this could affect models, Daniel plz double check}
Since \static text has no such feedback, \ptlms learn from all texts, as if they were all equally understandable by readers.
% \maarten{Potentially, can we make a third but succinct claim about how language primarily used for communication/interaction \cite{wells1981learning}; \static text is only one half of the speaker-listener dyad; and interactions allow for immediate feedback of whether what we're saying could/should be ajusted (i.e., perlocutionary aspects of language)? Daniel, if you could give that a go?}

\paragraph{Centering theory.}
% Yejin: Centering theory: surface text is gonna give information more on the person in the focus, and thus there will be more information on that person. 
% Learning to distinguish characters in \static text is challenging due to text often having a single focus or perspective.
At any given time, most text focuses on describing one protagonist and their relation to their surroundings, according to Centering Theory \cite{Grosz1995-hm}.
As such, main characters and their mental states are more likely to be \textit{described}, whereas other participants might only be \textit{mentioned}.
Additionally, main characters are more likely to be referred to with pronouns, whereas secondary characters with their names.
% According to Centering Theory \cite{Grosz1995-hm}, the centrality of a character in a discourse is often marked by their being referred to with pronouns, whereas secondary characters are often referred to by name.
Thus, a model trained purely on \static text might not learn to reason about social intelligence or mental states and realities of different characters of situations; they might not even inherently learn to resolve coreference for multiple characters \cite{sakaguchi2020winogrande}.
% resolve coreference for multiple characters inherently \cite{sakaguchi2020winogrande}, much less reasoning about social intelligence or mental states and realities of different characters of situations.


% \clearpage
\subsection{Future directions towards \ptlms with \TheoryOfMind}
\label{ssec:future-directions}

% \maarten{Something like: }
While there is no one best path towards \ptlms with social intelligence and \TheoryOfMind, it seems likely that this will require challenging the standard \ptlms paradigm of training on \static text with the language modelling objective.
Based on our findings and the limitations we discussed, we outline some possible directions forward below.
% Below, we outline some possible directions forward, focusing on person-centric and socially aware approaches.

% \paragraph{Beyond \Static Text as Training Data}


% 1. Better grounding in social context, similar to how it seems to helps in vision.
% 2. Entity-centric neural architectures

\maarten{Todo: Pepper in notions of what might be challenges to our proposed solutions/maybe lay out alternative solutions?}

% \maarten{Yejin: (1) interaction vs. interactive environments are not the same, and Y doesn't believe interaction will solve everything. \\(2) would be good to highlight some challenges that could arise / admit that we don't know what will work. \\(3) for entity-centric, discuss the differences between grounding text in a wiki-entity vs. actually reasoning about entity mental states (need to go a little further than what we say currently, i.e., that entity-centric will work) \\(4) question of challenges likely will fall on ``we don't have the data'' so if we can address that point better (gamification/guessing games? data ablation to force models to learn better? first pretrain on \static text and then finetune on social text?)}

\maarten{My restructuring ideas (will draw heavily from what is currently written): % endorsed by Y! woot haha
1. Maybe just changing the data will help the models learn ToM and social intelligence? What if data contained more elaborations of social commonsense, how characters feel, etc. Maybe that would teach the model everything it needs? However, a key component for language models seems to be the scale, which can make a big difference; so getting this kind of data at scale would likely take a long time. Possibly, we could use smaller amounts of data that has this information and finetune the PTLMs on that (or use RL); that has been known to work for \cite{Zhou2021PretrainingTT}.
2. So maybe we also need to add inductive biases to the model architecture / training objective; possibly, this could be done supervisedly, but again we don't have the data. So it would have to be done unsupervisedly. these could be inspired by neuroscience \cite{Langley2022-fl}, or could be based on investigations of what concepts neural models learn in latent ways through pretraining, and honing in on those in some ways. This would need more research, and could potentially require also returning to recurrent models. Also, this 
3. Maybe that's still not enough, and maybe models will never learn social intelligence from just reading text, regardless of what the text contains / whether it's \static or not. Maybe the only way to learn language will be through some sort of interaction paradigm \cite{Zhu2021-zj}, or emergent communication \cite{steinert2022emergent}. But these kinds of simulations etc. have limits too, and would require an open-world model of language , which is currently not real \cite{Ludwin-Peery2021-hx}. % there's no empirical success that any model out of simulation generalizes out of that simulation environment; all these models only learning the spurious correlations of the environment \cite{Ludwin-Peery2021-hx}.
4. Nevertheless, we need to keep building benchmarks for measuring theory of mind and social intelligence.
}
\daniel{yeah I like this framing/structure! And could add some stuff to go alongside the neuroscience (explicit pragmatic/ToM reasoning) if useful.}\maarten{Yes please}


\paragraph{Beyond \Static Text as Training Data}
% Due to these limitations, we posit that \ptlms could more efficiently learn \TheoryOfMind abilities through non-\static training data, entity-centric neural architectures and social training objectives.
Similar to how visual groundings can help with learning physical knowledge \cite{Zhang2022-nk}, grounding training data in its social context
(e.g., communicative intents, speaker identities) could enable better learning of \TheoryOfMind abilities.
% Echoing arguments by \citet{Bender2020-kt,Bisk2020-xb}, grounding the text used to train \ptlms in its social context (e.g.,  communicative intents, speaker identities) could enable better learning on \TheoryOfMind abilities.
Echoing arguments by \citet{Bender2020-kt,Bisk2020-xb}, this could be accomplished by exploring more interactional training data, such as dialogues in situated contexts that explicitly require reasoning about interlocutor mental states \cite{Bara2021-xd,Zhu2021-zj}. 
\maarten{Need to take this further, be more concrete, and say that learning during interaction is not the same as learning from interactional data? Also address the challenge of how to get the data?}
% \maarten{Challenge is getting this context/metadata then? Can we use the example from \cite{Zhou2021PretrainingTT} as an example that it may be fine to finetune PTLMs on better data to get them to exhibit \TheoryOfMind like abilities better?}

\paragraph{Entity-aware neural architectures}
However, changing the training data alone will likely not suffice for \ptlms to efficiently learn social intelligence and \TheoryOfMind; new entity-centric neural architectures are also required.
Humans are believed to have concept cells \cite{Bowers2017-hp,Calvo_Tapia2020-ll}, i.e., sets of neurons that activate for specific people or concepts; we theorize that this type of inductive bias could benefit social intelligence in \ptlms \cite[for a longer discussion of how neurological insights can help with AI \ToM, see][]{Langley2022-fl}.
Prior work has shown that recurrent neural architectures with explicit entity- or person-level representations and training objective can do well at entity identification and tracking tasks \cite{Henaff2017-ov,Ji2017-iq,Yang2017-uk,Liu2019-kn}, and more recent work has corroborated this with larger Transformer-based models \cite{Fevry2020-vm,De_Cao2020-ve,Rosset2020-bj}.
Beyond identification and tracking, \ptlms training could be augmented with tasks specifically related to \TheoryOfMind, such as those explored by \citet{Zhu2021-zj,Wang2022-vi}.
\maarten{Need to take this further, cause there's a big difference between identifying entities / grounding them in wikipedia vs. the model learning theory of mind... }

% Additionally, \TheoryOfMind training could be done after an initial pretraining on \static text, inspired by promising evidence that pretrained \ptlms better learn commonsense knowledge through additional pretraining on commonsense tasks \cite{Zhou2021PretrainingTT}.
% Such approaches would circumvent the need for augmenting massive corpora of text with social context (e.g., coreference labels, communicative intents).
% % \ronan{We could also include \cite[CALM]{Zhou2021PretrainingTT}, about ``self-supervised pre-training objectives in both generative and contrastive form to improve the commonsense reasoning ability of pre-trained text-to-text transformers''.}

% \maarten{Daniel, can you take a stab at this:}\daniel{Possible things to call for in future work: intrinsic evaluation / probing of ToM, beyond behavioral evals. Ongoing work has probed for semantics (maybe cite Belinda Li's paper \cite{Li2021-mp}), which may give a way to ground form-trained models to meaning, while requiring only a very small amount of form--meaning mapping. There are likely analogues of this for pragmatics / ToM.}

\paragraph{Person-centric training paradigm}
Beyond the data and architecture directions above, alternative training procedures for \ptlms could help produce \TheoryOfMind capabilities.
Recent work has found evidence for latent representations of grounded semantics in models trained only on \static text \cite{Li2021-mp}, which can be tied to real-world grounding with a small amount of additional training \cite{Patel2022-mapping}. %. %, \eg in semi-supervised pre-training or in fine-tuning.
Similarly promising experiments show that
% Additionally, \TheoryOfMind training could be done after an initial pretraining on \static text, inspired by promising evidence that 
pretrained \ptlms better learn commonsense knowledge through additional pretraining on commonsense tasks \cite{Zhou2021PretrainingTT}.
This latent variable perspective might also help to learn \TheoryOfMind:
we encourage future work to continue to probe for evidence of social and pragmatic representations in existing models, and consider additional human-in-the-loop or multi-agent pretraining and finetuning objectives to help surface and strengthen these capabilities, such as those explored by \citet{Hawkins2019-adaptation}, \citet{lazaridou-etal-2020-multi}, \citet{Zhu2021-zj}, and \citet{Wang2022-vi}.
% For theory-of-mind capabilities, 
% Beyond identification and tracking, \ptlms training could be augmented with tasks specifically related to \TheoryOfMind, 
Such approaches might circumvent the need for augmenting massive corpora of text with social context (e.g., coreference labels, communicative intents) while allowing models to learn the \TheoryOfMind capabilities necessary to aid communication and interact successfully with people.
% \ronan{We could also include \cite[CALM]{Zhou2021PretrainingTT}, about ``self-supervised pre-training objectives in both generative and contrastive form to improve the commonsense reasoning ability of pre-trained text-to-text transformers''.}


% Besides augmenting textual inputs with social context and adding entity-centric inductive biases to the neural architecture, the choice of the model's training objective and task could substantially enhance its social intelligence and \TheoryOfMind abilities.
% A model that only learns to predict the next word may learn to ignore entity-related cues due to the \static text limitations discussed above.
% However, multitask training on social intelligence tasks could improve the knowledge learned.



% We theorize that \ptlms would benefit from being trained on non-\static texts to learn \TheoryOfMind abilities.
% \maarten{I tried to write out some possible directions, but I started doubting myself. My struggles here: (1) GPT-3 was trained on some level of dialogues, cause it can clearly be a decent chatbot... yet it still does poorly... so training on the LM objective on dialogues may not solve the issue? Instead it may be that we need it to dedicate specific attention to entities/participants through different training objectives (2) has anyone actually shown that adding vision to your model is better than than text-only baselines at some sort of social task? \citet{Zhang2022-nk} show that vision-text LMs learn physical attributes better than text-only models, which I guess is cool / making the point I want to make?}

% \maarten{Thus, we argue that different types of data might be needed.
% Perhaps grounding in interactional data will be the answer \cite{Bara2021-xd}. 
% Or maybe models need to explicitly be taught social intelligence and pronoun resolution in addition to next word prediction.
% Additionally, echoing \cite{Bender2020-kt,Bisk2020-xb}, grounding in social context (e.g., social intents) could be helpful to enhance the social intelligence and \TheoryOfMind abilities of these models.
% }


% \daniel{A couple possible claims: (1) interaction is needed (2) interaction would be helpful (e.g., neural models could learn ToM in the limit, but might learn faster through interaction)}
% . \maarten{\Static text, i.e., text that is written for a general audience and is relatively self-contained, such as news articles, books, Wikipedia pages, is often written from an omniscient perspective: the reader receives most of the information needed, since it's content communicated exclusively through language (i.e., it's not often paired with visual or audio media).On the other hand, written text also omits obvious information, such as commonsense, because of grice's maxims.}

% \maarten{
% When it comes to learning about people from \static text, Centering Theory \cite{Grosz1995-hm} from pragmatics becomes relevant: often times, we use pronouns for protagonists but use people's names if they are not protagonists. This implies that it may be hard to learn mental state and person-centric realities that are useful for e.g., coref, cause we are often fed the person's name unless it's the protagonist.
% }


% \maarten{Daniel: for the discussion at the end, I wonder if you might consider going position-piece-y and speculating a bit on what interactive data that could help with ToM might look like (e.g., \cite{Bara2021-xd} ?). I don't have any great ideas for this now but would be excited to think about it!  I think this could complement B\&K and Bisk et al which like you said focused less on the social domains.}

% \subsection{Current training objectives and neural architectures are insufficiently person-centric}
% \subsection{Exploring person-centric model architectures and training objectives}
% \ptlms are mostly trained on the self-supervised language modeling objective, using stacked Transformer \cite{vaswani2017attention} layers.
% \maarten{Something about inductive biases for reasoning about 
% people more explicitly. Cognitively, we have concept cells \cite{Bowers2017-hp,Calvo_Tapia2020-ll}.
% Also, people have made LMs with specific entity representations \cite{Fevry2020-vm,De_Cao2020-ve,Rosset2020-bj}.
% Also good to discuss \cite{Langley2022-fl} -- a review discussing ToM and AI (have to read it)
% Also, discuss \cite{Wang2022-vi}, they introduce models/tasks that explicitly require ToM, and their model has explicit ToM-ness to it (guessing intentions, etc)
% Also cite Yonatan's paper \cite{Zhu2021-zj}, where they explicitly incorporate models of speakers/listeners and show that it helps in speaker-listener games.
% Echoing \citet{Bisk2020-xb}, the training objective is also an issue, in that it pushes low-tail things away; perhaps retrieval augmented training or decoding \cite[e.g., kNN-LM, REALM;][]{khandelwal2019generalization,guu2020realm}) should be part of the equation. Or maybe radically new objectives or paradigms are needed.
% }


% Specifically we show that these models lag far behind humans ($>$40\%) and behind finetuned models ($>$30\%) on the \socialIQa benchmark, which measure the commonsense reasoning abilities of models with respect to social interactions.

% \maarten{
% We showed that large pretrained LMs such as GPT-3 struggle with basic theory of mind capabilities in few-shot settings.
% Specifically, we show that these models lag far behind humans ($>$40\%) and behind finetuned models ($>$30\%) on the \socialIQa benchmark, which measure the commonsense reasoning abilities of models with respect to social interactions.
% Additionally, using the \tomi dataset, we show models struggle to distinguish between omniscient world knowledge vs. participant-centric world knowledge, lagging far behind human capabilities.
% We discuss some implications of our findings below.
% }

% Something about high-level re-iterating the issues with just pretraining on \static language.
% \maarten{
% Limitations of the paradigm of training only on the LM \textit{objective} on \static text \textit{data}.
% The issue with the data is that it may not contain enough information about participants, something something centering theory 
% Echoing arguments made by \cite{Bender2020-kt,Bisk2020-xb} on the limitations of learning meaning from pure form only (from pretraining on \static text), without grounding in physical or social context.
% } \ronan{+1}




% \maarten{Discussion with Ronan: 
% (1) \static text is typically omniscient narrator perspective, which is what the models probably have the most knowledge of?
% (2) probably need to say something about reporting biases and what is ommitted from \static text that might be needed to have ToM?
% (3) POssibly discuss the strawman of creating a robot-child that learns just from interaction
% }

% \maarten{Investigate: according to System Error, human brains have roughly 100B neurons , but today's biggest models are almost over that number?? According to further research, there's  100 trillion synapses in the brain which may be a better comparison -- GPT-3 is defs smaller in that case.}

% \daniel{Not directly in the scope of the datasets used here, but pragmatic meaning is often derived from reasoning about alternatives -- what the speaker could have said (in another context) but didn't. LLMs don't explicitly get access to these alternatives; they would have to piece them together across contexts.}\maarten{Added a comment above to incorporate}

% \daniel{Other things LLMs don't have access to (but again may be out-of-scope): seeing the perlocutionary effects of language; access to gestures, facial expressions, backchannels, acknowledgements, other features of discourse -- particularly face-to-face discourse -- that indicate uptake or understanding. Cite Clark \& Brennan 1991, or other common grounding literature.}


% \daniel{General ways to get inductive biases in model behavior: encode them in the data, in the architecture, in the loss function, or in intermediate representations. Some of these have been covered above, could there be others? Person-centric data augmentation?}


\section{Conclusion}
We explore the open question of whether and how much modern large-scale language models (\ptlms) can reason about social intelligence and \TheoryOfMind.
Our results show that out-of-the-box \ptlms struggle substantially with these abilities.
% Despite massive successes in other domains, our work highlighted some shortcomings of \ptlms at reasoning about social intelligence and \TheoryOfMind.
Specifically, \gptT's social intelligence as measured by \socialIQa lags behind humans (>30\%), and the model struggles to answer \tomi questions about mental states (55-60\%) compared factual questions (90--100\%).
In light of these shortcomings, we critically examine the large language model pretraining paradigm through the lens of pragmatics, and discuss possible directions towards enabling true social intelligence in NLP systems.
% We also saw that participant-centric reasoning is a particular challenge for \gptT.
% On \socialIQa, it often got participants of situations confused, and performed better for questions related to the main character of situations.
% With \tomi, \gptT performed increasingly worse from factual to first-order to second-order mental state questions.

==> old/2022-06-21-abstract.tex <==
% Tal Schuster's squib abstract
% Recent developments in neural language models (LMs) have raised concerns about their potentialmisuse for automatically spreading misinformation. In light of these concerns, several studieshave proposed to detect machine-generated fake news by capturing their stylistic differences fromhuman-written text. These approaches, broadly termed stylometry, have found success in source attribution and misinformation detection in human-written texts. 
% However, in this work, weshow that stylometry is limited against machine-generated misinformation. Whereas humansspeak differently when trying to deceive, LMs generate stylistically consistent text, regardlessof  underlying  motive.  Thus,  though  stylometry  can  successfully  prevent  impersonation  byidentifying text provenance, it fails to distinguish legitimate LM applications from those thatintroduce false information. We create two benchmarks demonstrating the stylistic similaritybetween malicious and legitimate uses of LMs, utilized in auto-completion and editing-assistancesettings.1Our findings highlight the need for non-stylometry approaches in detecting machine-generated misinformation, and open up the discussion on the desired evaluation benchmarks.

% NLP technology is increasingly used in tasks that require higher-order social intelligence
% Large PTLMs, where you learn to predict what word comes next based on previous words, are the backbone of many NLP systems these days.
% 

% \maarten{Todo: edit the abstract once we have a better story}

% Large pretrained language models (\ptlms) 
AI and NLP systems are increasingly deployed in settings that require complex social reasoning abilities.
AI and NLP systems require increasingly complex social reasoning abilities, as they are deployed in increasingly multi-user and user-adaptive settings.
% AI and NLP systems are increasingly used in complex social settings, such as to enhance communication between multiple people or to interact and adapt to users.
However, doing so effectively requires social intelligence and \TheoryOfMind (\ToM), i.e., the ability to reason about the different mental states, realities, intents, and reactions of all people involved.

In this work, we examine the open question of social intelligence and \TheoryOfMind in modern NLP systems from an empirical and theory-based perspective. % through empirical exploration and critical discussion.
We show that one of today's largest language models \cite[GPT-3;][]{brown2020language} lacks this kind of social intelligence out-of-the box, using two tasks:
% \maarten{Mention something about how people seemingly expect AGI to emerge from reading text? Or something about learning from predicting words?}
% In this work, we demonstrate that even today's largest language model \cite[GPT-3;][]{brown2020language} lacks this kind of social intelligence out-of-the box.
% To shed light onto this limitation, we analyze model performance on two tasks: %\ronan{Wondering if we should pitch it slightly differently, as this may sound as if we simply report the performance on two well-known benchmarks. Maybe more along the lines of: we analyze the performance and shed light on the limitations of current LMs?}\maarten{love it, added!}
\socialIQa \cite{sap2019socialIQa}, which measure models' ability to understand intents and reactions of participants of social interactions, and \tomi \cite{le-etal-2019-revisiting}, which measures whether models can infer mental states and realities of participants of situations.
% We show that models struggle on these social intelligence tasks, through comprehensive probing and question-answering experiments.

Our results show that models struggle substantially at these \TheoryOfMind tasks, with well-below-human accuracies of 55\% and 60\% on \socialIQa and \tomi, respectively. %, that lie well below human performance.
% Indeed, the best performance on \socialIQa reaches 55\% (>30\% below human performance), and accuracy on \tomi questions about mental states peaks at 60\% (30--40\% below accuracy on factual questions).
To conclude, we draw on theories from pragmatics to contextualize this shortcoming of large language models, by examining the limitations stemming from their data, neural architecture, and training paradigms.
Challenging the prevalent narrative that only scale is needed, we posit that person-centric NLP approaches might be more effective towards neural \TheoryOfMind.
% We conclude that increasing the scale of language models is likely not the most effective approach ,  that

% We discuss the implications and limitations of the current language modelling paradigm, \maarten{to update:} and posit that more interaction-oriented or participant-centric approaches to learning language are perhaps necessary.
% Our results suggest that learning language from static text alone will not endow models with social intelligence, and that perhaps more interactive or entity-aware approaches are necessary.

==> old/2022-06-21-background.tex <==
Before we examine the \TheoryOfMind abilities of \ptlms through language tasks, we first provide a brief summary of the \TheoryOfMind literature (\S\ref{ssec:tom-background}), as well as motivation for why \ptlms should have this type of social intelligence (\S\ref{ssec:why-ptls-need-tom}).

\maarten{Potentially, tie this in with Social Intelligence (see wikipedia article) too? Cause we're going broad.}
\subsection{Theory of Mind, Language, and Social Reasoning}\label{ssec:tom-background}
\TheoryOfMind (\ToM) describes the ability that we, as humans, have to ascribe and infer the mental states of others, and to predict which likely actions they are going to take \cite{apperly2010mindreaders}.%
\footnote{Note that, while Theory of Mind is well developed in most adults \cite{ganaie2015study}, reasoning and inference capabilities can be influenced by age, culture, neurodiversity, or developmental disorders \cite{korkmaz2011theory}.}
Most neuroscientists believe this ability develops in neurotypical children around ages 3 to 5 \cite{Wellman1992-zj}, although some work argues that preverbal infants already possess some level of \ToM-abilities \cite{Onishi2005-pm,Southgate2014-gi,Poulin-Dubois2018-td}.
One prominent theory of the functioning of \ToM is the \textit{mental simulation theory}, which posits that we create mental models of situations that we encounter and use those models to make inferences about the situation and its participants \cite{Graesser1994-cc,Heal1995-ns,Goldman2006-nb}.
We refer the reader to \citet{Langley2022-fl} for a recent review of the cognitive and neurological understandings of \TheoryOfMind.


% \footnote{There is also an increasing body of work showing some level of \ToM-type abilities in preverbal infants \cite{Onishi2005-pm,Southgate2014-gi,Poulin-Dubois2018-td}.} 
Relevant to our current study, there is evidence that language abilities and \ToM develop around similar ages in children \cite{Sperber1986-ha,Miller2006-pg,Tauzin2018-na}.
Through the lens of pragmatics, this link can be understood as the need for reasoning about an interlocutor's mental state in order to effectively communicate \cite{grice1975logic,Fernandez2013-su,Goodman2016-rsa,Enrici2019-mf}.
% \maarten{Debate about preverbal infants having tom \cite{Onishi2005-pm,Southgate2014-gi,Poulin-Dubois2018-td}.}

%Several theories have emerged as to how \ToM works and what the underlying processes are.
%A prominent one is the \textit{mental simulation theory}, which posits that we create mental models of situations that we encounter and use those models to make inferences about the situation \cite{Graesser1994-cc,Heal1995-ns,Goldman2006-nb}. 
% Those mental models are both influenced by our commonsense knowledge about the world as well as our own past experiences \cite{kintsch1988role,Conway2000-nl}.


\subsection{Why Large Language Models need \TheoryOfMind Reasoning}\label{ssec:why-ptls-need-tom}
Social intelligence, \TheoryOfMind, and commonsense reasoning have been a longstanding but elusive goal of artificial intelligence for decades \citep{Gunning2018-xn,Choi2022-sv}.
These reasoning abilities are becoming increasingly necessary as AI assistants are used in situations where they will require social intelligence and Theory of Mind in order to operate effectively \cite{Wang2007-xa,Dhelim2021-sd,Langley2022-fl}.
For example, new technologies are emerging where AI is used to \textit{interact} and \emph{adapt} to users \cite{Bickmore2005-relationships,Jaques2019-gp}, e.g., voice assistants, smart homes, and tutoring systems; or where AI helps \textit{enhance communication} between multiple users, e.g., email autocomplete \citep{Chen2019smartCompose}, AI-assisted counseling 
\cite{Kearns2020-ty,Allen2020-cd,sharma2021towards}, or facilitated discussion in online courses \cite{Rose2014-mooc-attrition}.

As we move beyond just asking single-turn questions to social and interactive AI assistants, % (e.g., about the weather),
higher order reasoning becomes necessary \cite{McDonald2019-fy}.
For example, AI systems should be capable of more nuanced understanding, such as ensuring an alarm is on if someone has a job interview the next morning \cite{Dhelim2021-sd}, 
knowing to call for help when an elderly person falls \cite{pollack2005intelligent}, inferring personality and intentions in dialogues \cite{Mairesse2007-personality,wang-etal-2019-persuasion}, reasoning about public commitments \cite{Asher2013-strategic-conversation},
predicting emotional and affective states \cite{litman-forbes-riley-2004-predicting,jaques-etal-2020-human},
and incorporating empathy, interlocutor perspective, and social intelligence \cite{Kearns2020-ty,sharma2021towards}.

% Additionally, as AI chatbots are being developed to help counselors, research has shown the importance of incorporating empathy, the interlocutor's perspective, and social intelligence \cite{Kearns2020-ty,sharma2021towards}.
% \maarten{Add some work by Natasha Jacques?} % daniel: added


% \section{\gptT: one of the Largest LMs as an Upper Bound on Neural \TheoryOfMind}
% To estimate an upper bound of \TheoryOfMind abilities of current neural models, we focus on the \gptT family of models \cite{brown2020language}, which contains one of the largest \ptlms in existence (\gptDavinci).
% Ranging from 125M to 175B parameters, the \gptT models were all trained on 499B word tokens of general web text (including general news, blogs, Wikipedia, and fan fiction books).
% Their training objective was to learn to predict the likelihood of a word given preceding words $p(w_{i+1}\mid w_{0:i})$, using a neural network of multiple layers of the Transformer architecture \cite{vaswani2017attention}.



% \gptDavinci is 175B parameter model, trained on 499 billion word tokens of general web text (including general news, blogs, Wikipedia, fan fiction books).
%To measure whether models can do \TheoryOfMind-style reasoning, we operate under the premise that larger models are likely more capable
%\maarten{Something about how their performance is quite impressive?}
%\maarten{Maybe add a few sentences on how LMs are trained?}
%\maarten{Not sure if we need this here? Though it could be a good place to quickly introduce GPT-3 and stuff? So just say that models are large NNs trained on the LM objective $p(w_{i+1}\mid w_0^i)$ using Transformer architecture \cite{vaswani2017attention}. }
